BeamSurfer: Minimalist Beam Management of Mobile mm-Wave Devices

Management of narrow directional beams is critical for mm-wave communication systems. Translational or rotational motion of the user can cause misalignment of transmit and receive beams with the base station losing track of the mobile. Reacquiring the user can take about one second in 5G NewRadio systems and significantly impair performance of applications, besides being energy intensive. It is therefore important to manage beams to continually maintain high received signal strength and prevent outages. It is also important to be able to recover from sudden but transient blockage caused by a handor face interposed in the Line-of-Sight (LoS) path. This work presents a beam management protocol called BeamSurfer that is targeted to the use case of users walking indoors near a base station. It is designed to be minimalistic, employing only in-band information, and not requiring knowledge such as location or orientation of the mobile device or any additional sensors. Evaluations under pedestrian mobility show that96%of the time it employs beams that are within3dB of what an omniscient Oracle would have chosen as the pair of optimal transmit-receive LoS beams. It also recovers from transient LoS blockage by continuing to maintain control packet communication over a pre-selected reflected path that preserves time-synchronization with the base station, which allows it to rapidly recover to the LoS link as soon as it is unblocked

==> Reviewer1.tex <==
\section{Response to Reviewer 1}
We thank the reviewer for the thorough review and feedback. 
% Our focus in the revised manuscript was to clearly state the novelties and contributions. We hope that you find the following response satisfactory. 
\\
\newline
\textbf{The acronym RSS looks unnecessary and can be avoided. } \\
Done. The acronym ``RSS" is not used any more.
\\~\\
\textbf{page 2: line 10: the word `than' may not be needed} \\
Done. Word ``than" deleted.
\\~\\
\textbf{Page 2: line 53: I think the statement ``Such a delay...applications'' is not well connected to the previous statement. Also, this statement is already made previously. So it may be unnecessary.} 
\\
Done. Sentence deleted.
\\~\\
\textbf{I suggest avoiding the acronym BW for beamwidth as people in communications are historically used to using BW for bandwidth.}\\
Done. Acronym ``BW" is not used any more.
\\~\\
\textbf{Page 7: line 18: By orientation, do the authors mean the vertical tilt of the mobile?} \\
Done. We have added clarification in Section ??, lines ??-?? on pages ?? that it refers to both vertical as well as horizontal orientation. 
\\~\\
\textbf{Page 7: lines 42-43: Is there any gain in BeamSurfer compared to Swift-link. The requirement that Swift-link needs a good training sequence may not be a major drawback in practice. Also, using compressive sensing is a nice idea in sparse settings like this.}\\
Done. A detailed comparison with not just Swift-link, but also FALP and HBA, is given in Section 1, {\color{red}lines ??-?? on pages ??-??}, as well as Section IX-D,  on pages ??-??. We also point out a role for compressive sensing in determining a NLOS beam in Section ??, lines ??-??, pages ??-??.
\\~\\
\textbf{Page 8: lines 29-30: It is not clear what the authors mean by `other arrays'.}\\
Done. We have clarified in Section ??, lines ??-?? on pages ?? that [34] suggests employing four antenna arrays placed at the four corners of the mobile, and elaborated on their suggested approach.
\\~\\
\textbf{Page 8: lines 41-46: What kind of sensors do [39] consider? Using sensors may be a good idea indeed since our mobile phones already have several sensors which are quite accurate.}\\
Done. See Section IV.B, lines ??-?? on pages ??-??.
% We have listed the specific sensors.
% We have also explained that the sensors cannot provide estimates that are sufficiently accurate, less than $1.2^\circ$ error, to correct beam misalignment. I THINK THIS SENTENCE WILL NEED TO BE SHARPENED. LET US DISCUSS THIS.
\\~\\
\textbf{Same explanations are repeated several times on lines pages 1-12, especially how the proposed BeamSurfer handles misalignment due to mobility and how it deals with blockage. I believe pages 1-12 can be effectively compressed to not more than 5-6 pages and yet say everything that has been said in these pages. I would suggest the authors do the same.
}\\
Done. We have eliminated some repetition in several sections.
% {\color{red}Professor, I am not sure how to address it, such compression might lead to misunderstanding the work }
\\~\\
\textbf{Page 18: using NO for normal operation may not be a good idea. Maybe authors can use N.Op or something else which makes more sense. } \\
Done. Changed NO to N.Op 
\\~\\
\textbf{Page 22: lines 2-4: the explanations for Fig. 7 and 8 seem to be mixed up.}\\
Done. We corrected the figure numbers.
\\~\\
\textbf{Fig. 8a: What is meant by  `random walk' in the experiment?  Also, the figure needs a clear explanation.}\\
Done. Random walk is described in Table ??, and its caption now provides full explanation.
\\~\\
\textbf{Page 23: Explanation for Figs. 10 and 12 seem to be mixed up.}
\\
Done. We corrected the figure numbers.
\\~\\
\textbf{ The  caption for Fig.  12 seems to be wrong}\\
Done. The caption has been corrected.
\\~\\
\textbf{Also, the explanation for Fig. 10 (which is written as Fig. 12 on page 23) is not clear. The explanation and figure do not seem to say the same thing. } \\
Done. 
\\~\\
\textbf{Also, I expect the random walk to be more detrimental in Fig. 10a. But it seems to show that the translational motion is has reduced throughput compared to random walk.}\\
What is presented in those figures is the CDFs of the Throughput, and a higher CDF indeed means lower performance.
(For example the CDF plot of children's height is above the CDF plot for adult heights).
Fig. 10a indeed shows that translational motion at 1.4m/s yields better throughput than random walk as the reviewer expects.
To make this clear to readers we have indicated the median throughput for each case. For Translational Motion, the median throughput is {\color{red}??}, which is indeed larger than the median throughput of {\color{red}??} for Random Walk. We have also indicated this in the caption to assist readers in interpreting the graphs. 
% {\color{red}SANTOSH: CAN YOU PLEASE INDICATE THE MEDIAN THROUGHPUT WITH A DOT AND LABEL IT AS MEDIAN THROUGHPUT IN THE LEFT GRAPH?} -- taken care.
\\~\\
\textbf{There are no comparisons with the previous works, which makes it difficult to judge the merit of the proposed method. I would suggest comparing the results with at least the compressive sensing-based methods, such as the Swift-link. }\\
Done. We have provided detailed comparison in Section 1, lines ??-?? on pages ??-??, and have added a new Section IX.D on detailed performance comparison with other methods.
% Please find performance comparison in Section  \romannumeral 9 on page xx.





==> Reviewer2.tex <==
\section{Response to Reviewer 2}
{We thank the reviewer for a thorough review, and urging us to present detailed performance comparisons. 
We have now done both in Section 1, lines ??-?? on pages ??-??, as well as added a new subsection on performance comparison with other methods as Section IX.D on pages ??-??.
% Our focus in the revised manuscript was to clearly state the novelties and contributions. We hope that you find the following response satisfactory. \\
\newline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{The authors can provide complexity and performance comparison of beam-surfer with beam-forecast, swift-link and HBA for a better exposition.}

Done. We have added this in two places: in Section 1, lines ??-?? on pages ??-??, as well as added a new Section IX.D on performance comparison with other methods along several dimensions as Section IX.D on pages ??-??. We have also indicated a potential role for compressive sensing methods for determining a NLOS beam in {\color{red}Section ??, lines ??-??, pages ??-??}.

\textbf{Can sampling strategies such as Thompson sampling in the spatial vicinity of currently selected beam be employed for beam selection to make the beam-adaptation/exploration faster?} \\
 { Done, see Observation 2 in Section VII.B. For a uniform linear array, there are only 2 possible neighbors beams. For the case of a uniform planar array also there may be only two neighbor beams if the steering is only in the azimuth direction as in our testbed, and a maximum of 8 neighbor beams if steering is in both the azimuth as well zenith directions.
  So the search space is small, and we just use a simple method of testing the few possibilities and choosing the best as noted there. If there is a posterior probability distribution then Thompson sampling or other random exploration or learning methods can be used. Other approaches are compared in Section {\color{red}Related work}}\\~\\
  
\textbf{When both the optimal Tx beam involves a reflected path, i.e., in NLoS operation, how are better beams selected over time?   The optimal reflected beam can keep varying over time (with or without the LoS blocked). Why are 3dB and 10 dB chosen as thresholds in the protocol? What are the effects of tweaking these thresholds? } \\
{
Done. 
% {\color{red} I don't believe we have succinctly answered the reviewer's question on ``When both the optimal Tx beam involves a reflected path, i.e., in NLoS operation, how are better beams selected over time?". Can you please give a succinct answer, referring the reviewer to the particular place in the manuscript where this is answered. Please see my comment in Point 5 in Section VI.}
% {\color{red} We have also not succinctly answered the reviewer's question on "The optimal reflected beam can keep varying over time (with or without the LoS blocked)". For this point we need to say how we are constantly searching for a good reflected beam and improving it."}
Done. We have indicated in Section IV.B in lines ??-?? on pages ??-?? that it is currently done by exhaustive search whenever the transmit beam changes, which we have found is sufficiently frequent to maintain a viable control channel, and that for further improvement one can also update each time the LoS receive beam changes, and to do so potentially using compressive sensing methods.
The reason for the 3dB threshold for
LoS is explained in Section IV.A, lines ??-?? on lines ??-?? on pages ??-??.
% Reason for choice of 3dB threshold described in Section IV.A, page ??. For convenience we reproduce that here. ``For the main lobe of an antenna radiation pattern, the directional gain drops steeply after half power, hence 3dB gain is chosen to reflect this and to utilize a beam only within its beam width (half power points) where the gain is maximum. Also, the first null beam width, i.e, angular width between zero gain points for a linear array antenna pattern is approximately twice beam width. So the antenna gain drops steeply after the half power point."
The reason for the 10dB threshold for NLOS is explained in Section IV.A, lines ??-?? on pages ??-??.}
% As described in Section IV.B, page ??, the choice for NLOS was based on extensive experiments in indoor environments such as classrooms, corridors, and conference rooms in our building, where we found that the usable NLoS RSS is within 10 dB of LoS RSS.
% {\color{red} Can you add any other reason for the choice of 10dB other than that it was best in your experiments? If so, please add to the paper too.}
}
\\~\\
\textbf{What are the factors affecting BCT? How can it be bounded in general for indoor/outdoor channels?}\\ 
{Done. 
See Section IV.A, lines ??-?? on pages ??-??.
% We have added the following in Section IV. Given a LoS path, a particular receiver beam can receive usable signal as long as LoS path remains within its receive beam width. 
% As the user moves, the LoS path moves out of beam width, and the duration after which the RSS drops below 3 dB from its maximum is the BCT. 
% So the primary factors affecting BCT are width of beam and user mobility. 
% Our experimental results for a 12 element phased array, presented in Section ??, pages ??-??, confirmed these are the main contributing factors in both indoor and outdoor channels. 
% Whether it is indoor or outdoor, communication requires either a LoS or NLoS path between Transmitter and Receiver. 
% Our observations present the empirical bounds observed for user mobility when a beam from 12 element phased array is used. It is hard to find general bounds as BCT depends on mobility, antenna orientation, beam width used. In our opinion, BCT should as seen as profile (like a Power Delay Profile, which varies from scenario to scenario) for a particular scenario but not as generic model based observation.  Also, we find such modelling as an interesting future problem and must be both exclusively and extensively studied.
\\~\\
\textbf{Given RSS vs time data, how is the BCT computed? What is the variance of the RSS within a BCT slot?}\\

Done. See Section ??, lines ??-?? on pages ??-?? where it is explained how the
BCT is computed, {\color{red} Santosh. Please point them to the sentence "The BCT is determined from the graphs in Fig. \ref{fig:1}.  as the time taken for the Received Signal Strength to decrease by 3dB from its maximum." that I have added.} and Section ??, lines ??-?? on pages ?? for the standard deviation of the RSS within the BCT. {\color{red} Please point them to the sentence "`` The standard deviation of the RSS within the BCT is .. "}
% {\color{cyan}
% As described in Section IV.A, When the transmitter and receiver beams remain unchanged during a particular user motion pattern, duration over which received signal strength remains within 3 dB from the maximum is BCT. 
% 
% Variance of RSS within BCT depends on beam pattern within the half power beamwidths, which in turn depends on the type of array as well. RSS also depends on user motion pattern. Antenna radiation patterns often doesn't have closed form expression and researchers usually rely on numerical analysis. Variance of received signal strength, therefore is calculated based on observations. For simple translational motion and using 12 element phased array, variance is 1.2635
\\~\\
\textbf{The observations (such as on BCT and spatial correlation of beams) and conclusions drawn seem quite dependent on the channel geometry. How can this be generalized? In an outdoor channel geometry with multiple mobile scatters/obstructions, it is not clear why these observations and conclusions could remain valid. These observations and conclusions seem quite critical for the protocol's performance.} \\
{
% It is true that BCT is dependent on mobility and beam patterns. It is better to empirically calculate the same for a given system in similar fashion as power delay profile of channel in a given environment which vary from scenario to scenario. As we know a given power delay profile or channel model can’t be generalized so is BCT. Similar to channel parameters like delay spread which varies based on environment, BCT can only be characterized for particular system and mobility pattern. 
% 
% Our experiments in outdoor environment didn’t find usable NLoS path from scatterers, that is channel is primarily dominated by LoS path. For either a LoS path or NLoS path, we found BCT depends on beam width and user mobility, what we present in our work are experimental observations for typical motion patterns. Our protocol performance is independent of BCT durations, protocol can be tweaked based on BCT measurements for any intended mobility model and beam pattern, just like one of many empirical channel power delay profiles and neither of them can really replace others.
% 
Done. Please see the added paragraphs in Section ??, lines ??-?? on pages ??-??.
{\color{red}Santosh: Please point them to the location  with the lines ``Our results are based on experimental data collected over 2 months at different times of day,... empirically calculate BCTs for such scenarios to tune parameters of the protocol.}
% the same for a given system in similar fashion as power delay profile of channel in a given environment which vary from scenario to scenario. As we know a given power delay profile or channel model can’t be generalized so is BCT. Similar to channel parameters like delay spread which varies based on environment, BCT can only be characterized for particular system and mobility pattern. 
% 
% To the best of our knowledge, our work is the first in consolidating extensive experimental data for BCT for human walk. and we believe our observations of BCT stand as cross validation for the parameterizing BCT.
% We intend to release the data sets to the community for researchers to fit the data to identify a model. 
% However, we believe that is work in itself.
} \\

\textbf{In Figs. 2a and 2b,  it is counter intuitive to notice that the RSS for D = 10m being always better than that of D = 5m, as one would expect the signal strength to drop with distance. Can this be reasoned?}\\
{Done. The reviewer is correct. The figures were earlier presented using different amplifier gains. We have now normalized all of them to use the same amplifier gain, and one can indeed see that RSS for 5m distance is indeed better than RSS over 10m distance.
% {\color{red} Santosh, I cannot understand this explanation? What is the y-axis of the graph? Can you please explain it to me orally? It needs to be rewritten to be succinct and super-clear.} We intend to present Fig 2a and 2b to reflect the change of RSS (not the absolute RSS) with time for a given motion pattern and distance than the true RSS. So, we adjusted receiver gains of our hardware to have similar RSS at 5m and 10m. We can either add text explaining the same or we present the true RSS mentioning the receiver gain employed at the distance and the TX power. Further, we request reviewer to consider the whenever we mention RSS not in absolute sense for the entirety of work, as we only focus on change in RSS.
}
\\~\\
\textbf{For a typical movement pattern, can the outage probability of beam-surfer be analytically characterized and rate guarantees be given?} \\
That remains a topic for future work.
It will require mathematical channel modeling, model of the environment, and mathematical modeling of motion including orientation of mobile, and will be an interesting topic for future theoretical work.
\\~\\
\textbf{It is not clear how the synchronization is performed in this setup.} \\
Done. This is explained in Section ??, lines ??-?? on pages ??-??.
{\color{red} Can you please insert the following two sentences into some appropriate place in the paper, and simply refer the reviewer to that place?}{The transmit waveform in our transceivers has a frame of 10ms duration split into 100 slots. We dedicate the first 4 slot to send Zadoff Chu sequence known to the receiver to acquire timing of the frame and thereby slots.}} 

































==> Reviewer3.tex <==
\section{Response to Reviewer 3}


{We thank the reviewer for the thorough review.\\
\newline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{How can a receiver know that the transmitted beam is misaligned?  Please clarify.}\\
{Done. A sentence is added in Section ??, lines ??-?? on pages ??-??. {\color{red} Please point them to the location where the sentences ``If neither of the beams $k-1$ or $k+1$ has a higher RSS, then the receiver requests the transmittter to try its neighboring beams." have been added.} The details are indicated in Section VIII, page 27, lines ??-?? on pages ??-??, as well as shown in the State Machine of Figure 5 for the node TBA (Transmit Beam Adaptation), and
the Flowchart of the protocol in Fig. 6 corresponding to TX Beam Adaptation.
% If the receive beam adaptation at user couldn't restore RSS within 3 dB then user requests Transmit beam adaptation.
}
\\~\\
\textbf{Considering the point 4 which is mentioned under the key experimental findings in page 11,
   authors should comment on the effect of error on the system performance, which may arise during
   refining the misaligned beams.} \\
 {In the extensive experimental evaluations conducted, in spite of all measurement and other errors, BeamSurfer is able to maintain received signal strength within 3 dB of what an Omniscient Oracle could possibly achieve in all the mobility scenarios studied. No algorithm can perform better than an Omniscient Oracle which always chooses the best beam, and so it is an absolute upper bound on performance, and generally unachievable. The maximum throughput loss compared to the oracle when signal strength is 3 dB lesser is around 30 $\%$.}
 \\~\\  
\textbf{ Is the presented beam management protocol, applicable for both TDD and FDD based
 systems? Authors please clarify this. } \\
 {The protocol is applicable for both TDD and FDD systems as it is based only on RSS.  We implemented protocol for TDD system.} 
\\~\\
\textbf{In the line 36 of page 26, it is written that “…..  schedules a set of beams with with ……. ”.
 Please correct this.} \\
{ Done}
\\~\\
\textbf{What will be the effect of imperfect channel state information on the presented beam
  management? Please clarify.} \\
  {BeamSurfer doesn't need channel state information as it only relies on received signal strength.} }











==> goalsbackup.tex <==
\section{The Goals and Challenges of Beam management}
% Beam alignment delay can significantly impact the link performance. 
In mm-wave communication systems, narrow beams are necessary to overcome high path loss. Supporting ultra-low latency applications is challenging when users are mobile, either due to translational/rotational motion that causes beam misalignment, or the human body that can cause blockage between base station and user. 
% Consistent high link throughput is desirable for applications like high resolution video streaming, virtual reality and online gaming, etc. 
Re-connection attempts caused by User Loss result in outages, in addition to high modem power consumption due to complex {re-acquisition} procedures. 
Unlike omni-directional communication systems where interference can corrupt signal and impact the Signal-to-Interference plus Noise Ratio (SINR), mm-wave systems using narrow directional beams are less susceptible to signal contamination from neighbor devices. Therefore, maintaining good signal strength is sufficient. Avoiding user loss and maintaining high signal strength are the primary goals of this paper.
% Poor receive signal quality can cause packet decoding failures, and subsequent re-transmissions greatly reduce the MAC layer throughput.  
% mobiles might use wider beams to reduce initial search space, but eventually need to identify a narrow and a good aligned beam to improve probability of success of initial random access procedure and to maintain the connection thereafter. 


% A solution tailored to a specific local environment would entail
% prior mapping of the environment and determining transmit-receive beam pairs 
% that are appropriate for each mobile location
% and orientation.
% % , orientation, human body position
% % relative to mobile, i.e., whether interposed between mobile user and base station).
% % This has two disadvantages.
% This requires out-of-band information
% from sensors to determine the mobile location and orientation.
% % , human body position
% % relative to mobile), posing sensing challenges with respect to human body position relative to LoS
% % between mobile user and base station. 
% It also requires tailoring to several base stations since mobile mobiles switch a good number of base stations every day. 
% % and are expected to work globally.
% Also, even within the same location, the scatterers may change from moment to moment.

We explore a totally in-band solution without requiring any
out-of-band sensors. The solution is based purely on information
normally acquired over the radio domain.
Fundamental questions to be answered for a solution to be feasible are:
\begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
\item Is it possible to predict when a currently working LoS beam will cease to work? \item When a LoS beam ceases to work, is there likely to be another good beam? 
\item If so, how does one determine what that next beam is? 
\item Can the determination of the next beam be done in time to make the switch, given that it may need back and forth communication and agreement between mobile user and base station?  
% While that may resolve the transmit beam of the base station, 
\item Can one choose the mobile's receive beam efficiently without significant overhead of testing beams? 
\item How to ensure that the mobile continually has nearly the best transmit-receive beam pair at all times? \item Can this be done for the use case of users walking in the proximity of a base station? \item What is the overhead of the adaptation scheme? 
\item Are there likely to be suitable reflected beams in indoor environments when blockage happens? 
\item Can the mobile determine a receive configuration for reflected beams in advance to be prepared for blockage? 
% \itemCan one efficiently determine a suitable reflected beam to revert to in case of blockage? Scanning and storing all reflected paths would involve high overhead. Unlike LoS there is no notion of "neighboring reflected paths" since reflections from beams $k-1$ and $k+1$ can be dramatically different. Can a mobile predict what will be a good reflected beams without sampling all reflected beams? \item How do  mobile user and base station reach agreement on what reflected transmit beam from the base station to use? 
% \item Can recovery to a reflected beam be done quickly in time to avoid user loss?
\end{enumerate}
\begin{comment}
{\color{red}We need to say somewhere that our reflected beam solution is only for outdoor environments.
Also say somewhere that mm-wave at the moment we need to show that walking mobility can be handled, and that more ambitious usage is well down the road.}
\end{comment}
% (xiii) How much is 
% effective are: (i) What is the RSS threshold to change a beam? (ii) What is the optimal interval with which a mobile should make RSS measurements both to sustain the link and conserve its battery (iii) how to recovery dynamically from a link outage?


% \textbf{why only for human walk}

To address all these questions, beginning in Section \ref{measurementsection}, we investigate the impact on received signal strength of user motion, since it lies at the heart of all the {issues as well as all the solutions}. 
% The knowledge of the deterioration of RSS with mobility is vital for effective beam management.  
It determines how long a particular LoS beam is viable, similar to the notion of channel coherence time in wireless channels. We may call this ``beam coherence time under mobility." 
It determines how long one may ``surf" a beam, i.e., stay on a beam, and how much time one has to find a next beam to surf.
Moreover, how the received signal strength of other candidate beams changes
determines the feasibility of switching at an opportune moment to another beam. Similarly, the change of received signal strength with beam direction is important. The overhead of searching for the best beam will be large if one has to track all beams for their signal strengths, but it is much smaller if the angularly neighboring beams $k-1$ and $k+1$ are the candidates for the next configuration.

To save power in traditional cellular networks, mobiles go to sleep, and wake up at scheduled information exchange epochs to listen to omnidirectional broadcasts. 
% The mobile conserves its battery by keeping the modem in sleep mode and occasionally waking up for paging messages. The wake-up mechanism is quick in traditional cellular networks as the signal is omnidirectional. 
In contrast, for mm-Wave networks, mobiles are obliged to track base station beams by periodically taking signal measurements even for scheduling control packets.  Examining temporal characteristics of beam changes is therefore necessary to identify the optimal measurement rate.  

The next issue is that the base station can only decide on what transmit beam to use if the mobile informs it. This requires bilateral communication. Such ``control channel" communication for beams and epochs must be conducted at agreed upon epochs. Hence a key issue for scheduling LoS beams is predictability on what beams to use next.

Investigating behavior of signal strength on reflected beams is also critical. The time interval in which the signal strength of a reflected beam is approximately constant is critical to recovering from blockage. It is the ``beam coherence time of the reflected beam" under mobility. 

The following are our key experimental findings:
\begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
\item For a given mobility scenario, there is a certain duration,
    which we call the Beam Coherence Time (BCT), for which a prior aligned  Transmit-Receive beam pair remains usable.  This BCT is typically greater than $100$ ms 
    even when the user rotates and interposes her face to block the LoS beams. Tables  \ref{table:1} $\&$ \ref{rotation}  present BCT for various motion patterns.
    BeamSurfer adapts  measurement intervals to this BCT to minimize probing or alignment attempts.
     \item When receive beam $k$ of the mobile gets misaligned, the adjacent receive beams $k-1$ and $k+1$ are a good starting point for re-aligning the beam. The heatmaps in Figs. \ref{fig:heatmaptrans} and \ref{rotationmeasure} present the signal strengths measured at the mobile on all receive beams, while the user is in motion. They reveal that adjacent beams are indeed good choices to restore received signal strength.
    %  that has become misaligned due to user mobility.
     \item When receive beam adjustment by the mobile is not enough to compensate for mobility, the
     transmit beam needs to be changed. If the transmit beam
     $n$ is misaligned, the neighboring transmit beams $n-1$ and $n+1$ pointed in the adjacent
     directions are good starting points for re-aligning the transmit beam. The snapshots of experiments during BeamSurfer beam adaptation in Fig. \ref{beamsurferalignmentresults} identify occasions of transmit and receive beam adaptation.
    \item It is fine to choose a slightly misaligned beam first and refine it to reach a near-optimal pair of transmit-receive beams, rather than exploring afresh for the best beam pair. 
    % {\color{red} Not sure if this particular claim needs this, or if you can do so, but it would be good if you can  mention the particular figure or experiment that shows this?} {\color{green} Professor, I would like to leave this without referring to anything as the above figures are taking care of our intention}
    % % that satisfies QoS requirements.
    \item The transmit beam used for LoS communication typically also has a reflected path with $8$ to $10$ dB lesser signal strength in indoor environments. The receive beam must be changed to pick up this reflected path. This is an adaptation that can be performed by the mobile without
    requiring any coordination with the base station.
    This makes it possible to recover from blockage, which can be initiated by the mobile. {Signal strength measured on all beams and presented as heatmap in Fig. \ref{blockagemeasurement}c during our LoS blockage experiments demonstrate the existence of usable NLoS paths.}
    \item  As is evident from our experiments in Section \ref{measurementsection}, transmit and receive beams need constant adaptation to sustain the link during rapid user movements. Similarly, the corresponding NLoS paths do change as well. Therefore, blockage recovery by switching to a reflected beam
    needs to be adaptive since
    the wireless environment is dynamic and the scattering changes rapidly  with motion.
    Because the BCT of reflected beams is greater than $100$ ms,
    it is adequate for the mobile to scan for a reflected beam every $100$ ms or every time the
    base station switches to a new LoS transmit beam, and store it for future usage.
    The receive beam so found for a transmit beam within the past $100$ ms serves as a fallback when blockage happens.
    \item While the received signal strength of the reflected beam is about $8$ to $10$ dB lower than the
    LoS beam prior to blockage, as observed in our experiments in Section \ref{Human Body Blockage}, it is still adequate to maintain
    connectivity. 
    % and to keep that in reserve as a fllaback
    % in case blockage happens. 
    % The best receive beam to receive a reflected beam still can receive the refelcted beam
    % To scan whether there is a reflected transmit beam arriving to the mobile user from a certain direction, the mobile needs to align its receive its beam in that direction. We show that it is not necessary to scan all reflected paths to determine a reflected beam to hold in reserve in case of blockage. While there is no notion of ``neighboring beams" we show that a machine learning based ``content addressable memory" can be used for predicting a receive beam direction to switch in case of blockage. This solution is only presented to show that the problem is solvable, by presenting at least one efficient solution. Future researchers can well propose other machine learning solutions for receive beam scanning.
    \item Such an already found reflected path can be stored by the mobile
    and used to recover seamlessly from an outage caused by blockage since control packets can still be communicated back and forth between mobile and base station over the reflected path. 
    \item 
    % There is typically a better transmit-receive beam pair for the pair that was blocked.
    Recovery from blockage to a better transmit-receive beam pair can therefore be performed seamlessly as long as control packets
    can be exchanged between mobile and base station.
\end{enumerate}

Based on this experimental evidence, we compose a near-optimal solution for beam management that can make use of available phased arrays on mobiles and base stations, 
% pre-defined search directions, beamwidths, beam pattern and 
applicable to any mm-wave network, whether WiGig or 5G with directional beams, to overcome pathloss and absorption. We detail the BeamSurfer solution in the rest of the work. We specifically describe how it can be implemented in 5G mm-wave standards, and present an evaluation of the implemented solution.

==> introductionbackup.tex <==
\section{Introduction}
% The fifth generation ($5$G) cellular and IEEE 802.11ay WiFi standards are designed to provide gigabit throughput, ultra low latency and a reliable wireless link. Operating bands of $5$G are divided into two frequency bands FR1 ($450-6000$MHz) and FR2 ($24250-52600$MHz) \cite{_2017_nr1}, while 802.11ay operates in the $57$ to $70$ GHz region\cite{_2012_status}. FR2 and $60$ GHz bands fall in the mm-Wave band which is particularly challenging because of its propagation characteristics and susceptibility to blockage.  


% Free space path loss (FSPL) at $28GHz$ for $10m$ distance of separation is $\approx84dB$ \cite{pathloss,_2018_study}. 
% In addition, high frequency bands
% also suffer from 
% % high penetration and 
% oxygen absorption incurring a loss of up to $15$  db/km \cite{pathloss} at ground level. 
% Overcoming high path loss requires high gain antennas at both transmitter and receiver, which can be provided by an antenna array. 
% % Therefore, it is common to find an array of antennas in these devices. 
% % Using array gain to overcome high path loss however increases the  directivity of the transmission. 
% However, while the gain of the array increases with the number of antenna elements, the beamwidth of the pattern decreases. For a uniform linear array with $64$ elements, the beamwidth can be as narrow as $1^{\circ}$. 
% Therefore, mm-wave communication systems typically involve electronically steerable highly directional phased array antennas at both transmitter and receiver.
Millimeter wave communication systems require narrow radio beams to combat high path loss, e.g., free space path loss of $84$  dB at $28$ GHz at $10$ m and penetration loss of at least $8$ dB from common building materials \cite{pathloss,_2018_study}. 
% distance of separation 
% In addition, high frequency bands
% also suffer from 
% % high penetration and 
% oxygen absorption incurring a loss of up to $15$  db/km \cite{pathloss} at ground level.  (

{\color{red} page 2: line 10: the word `than' may not be needed.}
Ensuring that both receiving and transmitting beams are aligned ``towards each other" {\color{red}than} while a receiver is mobile is one of the major challenges for mm-wave devices since misalignment results in weak received signal strength (RSS). 
% from the network.
A second major challenge 
is blockage of the LoS path that can happen without warning, e.g., by a user suddenly rotating and interposing her hand or face between transmitter and receiver.
%  Blockage, especially by the human body, 
It results in a rapid loss of signal strength of at least $10$ dB \cite{collonge_2004_influence}, shown in Fig. \ref{blockagemeasurement}c,
immediately resulting in
% As mm-wave communication systems utilise high bandwidth, reduced RSS results in 
poor Signal to Noise Ratio (SNR) 
% {\color{red} Is there a reason you mention SNR in the case of blockage, but not in the case of mobility? \color{green}{Professor, although this is the case for both mobility and blockage, I felt it is more relevant in blockage, as link SNR diminishes almost instantaneously
% }} 
which leads to throughput degradation, increased packet re-transmissions, 
and possibly outage.
% Such blockage can easily happen if a user rotates, . 
%  antenna{\color{green}beam?}.
% When the mobile loses track of a transmit beam of the base station, it suffers a temporary service disconnection.
% Maintaining a link between a mobile mobile and transmitter requires both transmit beam and receive beam adaptation.
% For simplicity of exposition, we focus below on downlink where the base station is the transmitter and the user is the receiver, since by reversing transmission and reception the same pair of beams also works for uplink. 
Whether due to misalignment or blockage, if communication between base station and user is disrupted, then the mobile is ``lost" to the base station, and has to be re-acquired as a new user, which incurs a delay of about one second, impairing applications.

%{\footnote{Communication between base station and a particular user in cellular networks, especially for signal quality measurement reporting \cite{_2017_nr3} and control information \cite{_2017_nr2} exchange, takes place along a sequence of agreed upon ``epochs." 
% (In between these epochs the base station is busy communicating with other users or acquiring new users).
The base station and mobile communicate with each other in what may be called  ``communication epochs", which are time intervals where the sender and the receiver are simultaneously using the appropriate transmit and receive beams, respectively, for each other, i.e., ``pointed" at each other. In each such communication epoch they can also make ``appointments" for a limited number of future communication epochs, so that they can continue to maintain communication with each other in the future. If communication between base station and mobile does not take place at the next few epochs, then the mobile is effectively ``lost" to the base station
because the
mobile loses time synchronization with the base station,
and also the base station and mobile do not know which transmit-receive beam pair will be effective in to communicating after a delay.
The mobile will therefore need to be re-acquired all over again as a new user.
For acquiring new users,
mm-wave cellular base stations periodically transmit 
synchronization and reference signals.
% to facilitate a user's acquisition of the transmitter beams  within its sector. 
In 5G New Radio technology, every $20$ ms, 
a synchronization signal block (SSB) 
% with signals to acquire timing, cell identity, and broadcast information, 
is swept in up to $64$ directions \cite{_2017_nr2}. The acquisition delay can therefore be up to $1.28$ seconds for a mobile with single antenna array that is time unsynchronized with the base station, causing
% for a user with single antenna array. Thus losing the user 
% % causes a major performance impairment, which
% causes 
a significant performance hit 
for
% significantly impacts 
applications.
% running over mm-wave networks. 
Re-acquisition also drains power from the mobile \cite{huang_2012_a,saha_2017_a}.
Avoiding \enquote{connection loss} is the primary goal of a beam management protocol.
{\color{red}Page 2: line 53: I think the statement ``Such a delay...applications'' is not well connected to the previous statement. Also, this statement is already made previously. So it may be unnecessary.}

{\color{red}Such a delay of one second disrupts applications. Can we remove this line?}

% {\color{red}SANTOSH: OR SHOULD I JUST SAY LOSS HAPPENS WHEN THE BASE STATION DOES NOT KNOW WHICH TRANSMIT BEAM TO USE? }{\color{green} I think the current sentence is conveying our intention professor}
% However, this can incur a delay of the order of one second, significantly impacting the application running at the user.
% When a user is lost, it 


% Existing works on mm-wave beam management as presented in Section \ref{Related work} explored several solutions. All these solutions are either a overkill or out of band, meaning outside the mm-wave radio domain. Those solutions also have several  practical, delay and hardware complexity related shortcomings. 
{BeamSurfer targets the use case of users walking near a base
station. It employs two different mechanisms to avoid loss, one for
user mobility which requires continuous adaptation, and another
for blockage which is sudden and unpredictable.
It is a minimalist\footnote{The design philosophy of \enquote{less is more}, coined by Mies Van Der Rohe \cite{wiki:xxx}, is popular in the field of Architecture \cite{kim_2006}.
The architecture of mobile phones, especially the software and user interface, has embraced minimalist design from the
early 2010s.} solution in that it is a
totally in-band solution that uses the least amount of available information for minimizing connection loss due to either user mobility or blockage, requiring no other knowledge such as location or orientation. Yet, it is effective, as we show experimentally that {$96\%$ of the time} it employs transmit and receive beams that are within $3$ dB of what an omniscient Oracle would have chosen.
}

% , the main envisaged deployment of mm-wave networks.
BeamSurfer's 
% mobility adaptation mechanism and blockage recovery mechanism can be used for users walking indoors. 
% The 
mobility adaptation mechanism can also be used for users walking outdoors, but not its blockage recovery mechanism. The reason is that BeamSurfer harvests a reflected beam for blockage recovery, which generally does not exist outdoors.

\subsection*{Outline of mobility adaptation}
We outline the adaptation mechanism for mobility; the details of the full protocol are provided in Section \ref{beamsurfersection}.
In each communication epoch both the sender and the receiver need to know what transmit or receive beams to use. For clarity of discussion, we suppose that the base station is the sender and the mobile is the receiver. 
% By reciprocity, the same beams also work for communication in the reverse direction. 
The mobile need not reveal its receive beam to the base station. However, it needs to know that transmit beam the base station will use, which requires communication between them.

 As a user moves, BeamSurfer  adapts the mobile's receiving beam, and also enables timely adaptation of the base station's transmit beam.
% so that the RSS at the mobile is always within $3$ dB of the best pair of transmit-receive beams. 
It switches the beams so that the RSS at the mobile is always within $3$ dB of the best pair of transmit-receive beams
% to always stay within $3$ dB of the best pair of transmit-receive beam 
-- that is, it maintains receive gains within the peaks of the main lobes of the aligned beams. 
\begin{comment}
This is visualized in Fig. \ref{beamsurfer}.
\begin{figure}[h]
  \centering
  \includegraphics[width=.8\linewidth]{beamsurfermain.PNG}
  \caption{BeamSurfer switches TX and RX beams as the User moves}
  \label{beamsurfer}
\end{figure}
\end{comment}
% We elaborate further. 

{\color{red} I suggest avoiding the acronym BW for beamwidth as people in communications are historically used to using BW for bandwidth}

Each beam has a beamwidth {\color{red} $BW$ remove?}, defined as twice the angular deviation at which there is a $3$ dB loss from the maximum received signal strength. The experimental results presented in Sections
\ref{Lateral Translational Motion} and
\ref{Rotational Motion}
show that the gain outside one beamwidth of the main lobe of a beam drops significantly and is unpredictable.  The number of non-overlapping beams covering a $120^{\circ}$ sector is $N:= \frac{120}{BW}$ {\color{red}$N:= \frac{120}{Beamwidth}$?}. Let us order them as $1,2, \ldots, N$. Suppose the current best beam is beam $k$. After mobility over a time period of the order of tens of milliseconds, experimental results show that the next best beam is either beam $k$, $k-1$ or $k+1$ mod $N$, depending on whether the user continues moving/rotating in the same direction or changes direction. 
% This is true even if the user suddenly changes direction of motion. 
Section \ref{measurementsection} provides more details with measurement data for different motion patterns. BeamSurfer detects this $3$ dB loss, and employs an adaptation mechanism to determine which of beams $k-1$ or $k+1$ is the appropriate beam to switch to. Thereby, BeamSurfer ``surfs" the peaks of the transmit and receive beam lobes. The experimental evaluation of the performance of BeamSurfer in handling misalignment caused by mobility shown in Fig. \ref{beamsurferalignmentresults}.

Determining the best transmitting beam of the base station requires the adaptive mechanism to coordinate with the base station and mobile, while determining the user's best configuration can be done by itself without any coordination. 
The adaptive mechanism employs bilateral communication, as needed, and completes its decision making in a timely manner compatible with user mobility, to effectively switch beam pairs.

While we have
focused on downlink where the base station is the transmitter and the user is the receiver, if reciprocity holds, then, by reversing transmission and reception, the same pair of beams also works for uplink. 
In all our experiments, we found that beams are reciprocal, meaning a receiving beam is good for transmitting as well, so the same beam can be used for both uplink and downlink. Even for potential non-reciprocal scenarios, the mobility adaptation can remain the same with BeamSurfer's mechanisms remaining unchanged, except that separate beams will be needed for uplink and downlink.  

 The adaptation mechanism is completely in-band. It specifically requires no out-of-band information on location, pose, or any other side information \cite{citation01,citation02,citation03,citation04,citation05}. Unlike many alignment algorithms in the literature, BeamSurfer does not require the angle of arrival/departure estimates \cite{aod1,aod2,aod3} for beam alignment. Hence it can utilize  any 
 available beam patterns of a phased array \cite{phased_array}, and is applicable to any mm-wave technology.

% The adaptation mechanism switches both the base station's beam, but also the user's beam. the next beam switch,  and switches to the as a user moves the best beam As the user moves, BeamSurfer ``surfs" the peaks of the beams; It switches after every beamwidth, which corresponds to a 3dB loss, to another beam; hence the namethat the base station can use. For line of sight communication, the 
% As shown in Figure {\color{red} NUMBER} it switches from one near-optimal beam to the next one, ``surfing" along their peaks of signal strengths.
% It does not require any out-of-band information on user location or orientation. It also involves minimal overhead to surf along the running max
% of the available beams,succeeds in maintaining a beam that is always within 3dB of the optimally alogned pair of beams. boafter a successful connection establishment using one of its beams, the mobile constantly tracks signal quality on the same and switches to a different beam when necessary. As mentioned before, signal quality is primarily impacted by user mobility and blockage.

\subsection*{Outline of blockage recovery}
It is critical to avoid loss of the user for temporary blockages caused by an interposed hand or face between transmitter and receiver. 
Such blockage occurs suddenly, and so a different mechanism is needed to recover from transient blockages. (It is not possible to recover from permanent blockage except by handoff). 
% {\color{green} Depending on the motion and location of mobile, blockage can be temporary or long term, while link performance can be recovered for transient blockage and that is not the case for prolonged blockage } 
The key to recovery is to preserve time-synchronization
during blockage.
The BeamSurfer protocol pre-scans and stores receive beam identities for a good reflected path.
% and uses them to rapidly restore a link as soon as blockage happens.
Upon the sudden onset of blockage, BeamSurfer
 switches communication seamlessly to the pre-discovered good
reflected beam, which experiments show
has sufficient signal strength to  maintain connectivity and provide bidirectional communication with low-order modulation schemes for control packets.
This makes possible the critical functionality of preserving time-synchronization
during blockage.
% Otherwise the user will have
% to be reacquired, which incurs an outage of the order of one second.
It also makes it possible for the mobile to rendezvous back with the
base-station over an LoS path when the blockage ceases.
% Since communication interruption by blockage is unpredictable, the
% adaptive mechanism of SIN
% determines and stores a good reflected beam to switch to, in advance of blockage.

The solution presented is based on indoor experimental results
presented in Section \ref{Human Body Blockage}
that show that the same transmitting beam
already being used by the base station for line of sight (LoS) communication with the user typically also
reaches
the user along a reflected path
with signal strength about $8$ to $10$ dB less than the LoS beam.
% {\color{red}Your evaluation results show 10dB less} {\color{green} it is around 8 dB professor, it looks like 10, but it is 51 Los and 59 NLOs} lesser RSS.
This reflected beam can be updated every $100$ ms and stored for use
in case blockage occurs.
The experimental results of Section \ref{Human Body Blockage} show that it remains viable for that amount
of time even under mobility of the user. That is, the ``coherence time of reflected beams," defined more precisely in {Section \ref{Beam Coherence Time}}, is greater than $100$ ms. 

The user however needs to determine which is the best receive beam
that can pick up this reflected path.
This can be determined by scanning over all receive beams at a time that the base station is transmitting over the same transmit beam.
Such opportunities arise because the base station periodically
sweeps over all transmit beams at
pre-announced times to acquire new users. 
 Knowing this schedule, and being already time-synchronized with the base station, the mobile can scan over all its receive beams at the exact same time 
that the same transmit beam is being
used by the base station to acquire new users.
Such dual usage of beams will avoid using up valuable base station time.  
% usage of beams that will anyway be transmitted frequently, avoids using up valuable base station time.

While the signal strength of the reflected path is $8$ to $10$ dB lesser than for LoS, it is still
adequate for decoding control packets,
since those are transmitted by 
low order modulation schemes with polar or LDPC coding.
%{\footnote{In 5G NewRadio, QPSK is used with Polar coding.}}
(In addition, it can also sustain data at a smaller rate up to $1$ Mbps).
The control plane messages can then be used to coordinate recovery from blockage by initiating a search for the best pair of transmit-receive beams over a reflected path.
% Our experimental results indicate that such
% a better reflected path 
% over a different transmit beam does
% typically exist.

% Maintaining control connectivity allows efficient discovery of the
% appropriate transmit receive beam pair with a better reflected path.
% The above strategy of advance determination of a receive beam
% that can maintain control connectivity with the base station over a reflected path
% is used by Beam Surfer for Blockage Recovery.
% It does so without requiring the base station to change its transmit beam, as
% is desirable since it is only the mobile that knows that the blockage has occurred.

Prior works \cite{reflect2, reflect3} backed by extensive measurement campaigns have already shown that mm-wave frequencies reflect from various surfaces and the reflected paths are usable for communication.  
The following two experimental results described in Section 
\ref{Human Body Blockage} constitute additional properties of reflected beams in an indoor environment that enable BeamSurfer's blockage recovery mechanism described above:
% These make possible the above SIN mechanisms for blockage recovery. 
\begin{enumerate}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]
\item
The LoS transmit beam that is in current use 
typically also travels along a reflected path in the indoor environment, and
can be picked up by an appropriate receive beam with
signal strength that is no more than $10$ dB lesser than that of the LoS beam.
% This is important for two reasons, both of which
% are exploited in the BeamSurfer protocol.
Therefore, it is not necessary to switch the transmitting beam to overcome blockage.
The reason is that 
reversing the reflected path allows the user to communicate with the base station after a blockage happens.
This is critical since the base station does not know that blockage has occurred, and so cannot change its transmit beam. It is only the mobile that knows that the blockage has occurred, and it needs to initiate blockage recovery. The signal strength of the reflected beam is sufficient to sustain such control plane communication.
% using the same beam of the base station.
\item
The receive beam that can pick up the reflected path remains viable for at least $100$ ms, so it can be determined by the mobile
ahead of blockage and stored.
\end{enumerate}
% BeamSurfer's design for blockage recovery is built upon
% these experimental observations.
Fig. \ref{blockagerecovery} shows the ability of BeamSurfer to react successfully to blockages in a typical office room environment.

% In between 
% that there exists a multiplicity 
% of reflected paths in the mm wave band, and that
% the best of these reflected beams is typically of { $6$ to $8$ dB} less signal strength than LoS beams. This is sufficient to decode
% control packets which are transmitted by BPSK over Polar Coding. {\color{green} as it is mentioned earlier, a minor rephrasing, for control information exchange necessary for beam management?}
% Hence it can be used to efficiently initiate a search for the best transmit beam for the mobile.
% While the data rate is correspondingly 
% smaller, it nevertheless preserves connectivity between base station and user allowing them to coordinate on efficiently scheduling the next epoch so that the user is not lost.

% The protocol therefore functions by scanning receive beams reflected beams to see if they can pick up the current transmit beam in between epochs, the
% user monitors for reflected beams and their signal strengths.

% This mechanism requires bilateral communication which must take place in protocol specified time-slots, and the rescheduling of beams is accomplished in a way that it is accommodated in the latest 
% {\color{green}3GPP Release 15 Standard}.



% blockage occurs suddenly, the user commThe receiver beam adaptation primarily helps to overcome mobility and bl
% ockage. Whereas transmitter beam adaptation ensures coverage within the entire sector. User Mobility can be handled by timely switching of transmitter and receiver beams but blockage gives no warning and needs an instantaneous fallback non line of sight (NLoS) beam to maintain connection.


 A well-founded beam management strategy needs to be of low complexity, have small realignment delay, provide good RSS/SNR, and maximally avoid disconnection from the network.
% so as to handle mobility and blockage. 
%  We first experimentally characterize the impairments of user motion on RSS
%  in the sequel, and show that the above twin strategies 
%  to adapt to user mobility, and 
%  a dynamic recovery mechanism for link outage due to blockage, 
 BeamSurfer attains the above requirements
%  It 
% ensures good receive signal strength at the mobile. The evaluations results show
% that as intended in the design for adapting
% to mobility, it at all times chooses a transmit-receive beam pair that is within $3$ dB of the best transmit-receive beam pair that could be chosen by an oracle.
% As shown in Fig. \ref{BeamSurfer's handling of misalignment during user mobility}. {\color{red}SOMEHOW THE FIG NUMBER DOES NOT SHOW UP}, it adapts to the best aligned receiver beams  and triggers transmit beam adaptation when necessary. 
% %  It requires minimal measurements for relfected beams, and in consequence conserves device power. 
%  For handling blockage, BeamSurfer takes advantage of transmit beams already being broadcast by the base station to acquire new users, to determine a good reflected beam that can be used to sustain
%  control plane traffic. This allows it to seamlessly  initiate a process to determine the best transmit-receive pair post blockage.  
%  BeamSurfer achieves the above 
 by only employing
  data obtained during normal operation, {i.e., received signal strength}.
 
%  To recover from blockage, BeamSurfer harvests reflected paths dynamically, creates a binary content addressable memory, and uses them to restore the link. 

In the remainder of the paper, we first elaborate on the experiments in Section \ref{measurementsection}. Then we present BeamSurfer's design to adapt to mobility and to handle blockage in Section \ref{beamsurfersection}. To demonstrate robust performance
of the protocol, we have implemented it
on a software defined radio testbed working at $60$ GHz. 
The testbed, described in Section \ref{testbedsection}, has an electronically steerable phased array with narrow and wide beam code books that can scan either horizontally or full-space. 
These code books closely mimic commercial mm-wave modems. 
% both narrow/wider horizontal and full-space beam-codebooks, and closely mimics commercial mm-wave modems. 
We have performed experiments in both indoor and outdoor environments to study both LoS as well
as reflected, i.e., non line of sight (NLoS) paths.
% , and with  scatterers to study the nature of non-line of sight paths. 
We present the
results of extensive mobility experiments employing BeamSurfer in Section \ref{Implementation and Evaluation}.

==> reviewer1-1.tex <==
%\section{Response to Reviewer 1}

\textbf{Response to Reviewer 1} \\


We thank the reviewer for the thorough review and feedback. 
% Our focus in the revised manuscript was to clearly state the novelties and contributions. We hope that you find the following response satisfactory. 
\\
\newline
\textbf{The acronym RSS looks unnecessary and can be avoided. } \\
Done. The acronym ``RSS" is not used any more.
\\~\\
\textbf{page 2: line 10: the word `than' may not be needed} \\
Done. Word ``than" deleted.
\\~\\
\textbf{Page 2: line 53: I think the statement ``Such a delay...applications'' is not well connected to the previous statement. Also, this statement is already made previously. So it may be unnecessary.} 
\\
Done. Sentence deleted.
\\~\\
\textbf{I suggest avoiding the acronym BW for beamwidth as people in communications are historically used to using BW for bandwidth.}\\
Done. Acronym ``BW" is not used any more.
\\~\\
\textbf{Page 7: line 18: By orientation, do the authors mean the vertical tilt of the mobile?} \\
Done. We have added clarification in Section \RomanNumeralCaps{2}-A, lines 25-29 on page 6 that it refers to both vertical as well as horizontal orientation. 
\\~\\
\textbf{Page 7: lines 42-43: Is there any gain in BeamSurfer compared to Swift-link. The requirement that Swift-link needs a good training sequence may not be a major drawback in practice. Also, using compressive sensing is a nice idea in sparse settings like this.}\\
Done. A detailed comparison with not just Swift-link, but also FALP and HBA, is given in Section \RomanNumeralCaps{2}, on page 7, as well as Section \RomanNumeralCaps{9}-D,  on pages 22-24. We also point out a role for compressive sensing in determining a NLOS beam in Section \RomanNumeralCaps{1}-B, lines 13-15, pages 5.
\\~\\
\textbf{Page 8: lines 29-30: It is not clear what the authors mean by `other arrays'.}\\
Done. We have clarified in Section \RomanNumeralCaps{2}-A, lines 6-13 on page 8 that reference [36] suggests employing four antenna arrays placed at the four corners of the mobile, and elaborated on their suggested approach.
\\~\\
\textbf{Page 8: lines 41-46: What kind of sensors do [39] consider? Using sensors may be a good idea indeed since our mobile phones already have several sensors which are quite accurate.}\\
Done. See Section \RomanNumeralCaps{2}-B, lines 23-26 on page 7.
% We have listed the specific sensors.
% We have also explained that the sensors cannot provide estimates that are sufficiently accurate, less than $1.2^\circ$ error, to correct beam misalignment. I THINK THIS SENTENCE WILL NEED TO BE SHARPENED. LET US DISCUSS THIS.
\\~\\
\textbf{Same explanations are repeated several times on lines pages 1-12, especially how the proposed BeamSurfer handles misalignment due to mobility and how it deals with blockage. I believe pages 1-12 can be effectively compressed to not more than 5-6 pages and yet say everything that has been said in these pages. I would suggest the authors do the same.
}\\
Done. We have eliminated some repetition in several sections.
% {\color{red}Professor, I am not sure how to address it, such compression might lead to misunderstanding the work }
\\~\\
\textbf{Page 18: using NO for normal operation may not be a good idea. Maybe authors can use N.Op or something else which makes more sense. } \\
Done. Changed NO to N.Op 
\\~\\
\textbf{Page 22: lines 2-4: the explanations for Fig. 7 and 8 seem to be mixed up.}\\
Done. We corrected the figure numbers.
\\~\\
\textbf{Fig. 8a: What is meant by  `random walk' in the experiment?  Also, the figure needs a clear explanation.}\\
Done. Random walk is described in Table \RomanNumeralCaps{3}, and its caption now provides full explanation.
\\~\\
\textbf{Page 23: Explanation for Figs. 10 and 12 seem to be mixed up.}
\\
Done. We corrected the figure numbers.
\\~\\
\textbf{ The  caption for Fig.  12 seems to be wrong}\\
Done. The caption has been corrected.
\\~\\
\textbf{Also, the explanation for Fig. 10 (which is written as Fig. 12 on page 23) is not clear. The explanation and figure do not seem to say the same thing. } \\
Done. 
\\~\\
\textbf{Also, I expect the random walk to be more detrimental in Fig. 10a. But it seems to show that the translational motion is has reduced throughput compared to random walk.}\\
What is presented in those figures is the CDFs of the Throughput, and a higher CDF indeed means lower performance.
(For example the CDF plot of children's height is above the CDF plot for adult heights).
The figure, now numbered Fig. 9a, indeed shows that translational motion at 1.4 m/s yields better throughput than random walk as the reviewer expects.
To make this clear to readers we have indicated the median throughput for each case. For Translational Motion, the median throughput is 1.95 Gbps, which is indeed larger than the median throughput of 1.91 Gbps for Random Walk. We have also indicated this in the caption to assist readers in interpreting the graphs. 
% {\color{red}SANTOSH: CAN YOU PLEASE INDICATE THE MEDIAN THROUGHPUT WITH A DOT AND LABEL IT AS MEDIAN THROUGHPUT IN THE LEFT GRAPH?} -- taken care.
\\~\\
\textbf{There are no comparisons with the previous works, which makes it difficult to judge the merit of the proposed method. I would suggest comparing the results with at least the compressive sensing-based methods, such as the Swift-link. }\\
Done. We have provided a comparison in Section \RomanNumeralCaps{2}, and have added a new Section \RomanNumeralCaps{9}-D on detailed performance comparison with other methods. 
% Please find performance comparison in Section  \romannumeral 9 on page xx.





==> reviewer2-2.tex <==
%\section{Response to Reviewer 2}


\textbf{REVIEWER -2} \\



{We thank the reviewer for a thorough review, and urging us to present detailed performance comparisons. 
We have now done both in Section II, page 7, lines 4-32, as well as added a new subsection on performance comparison with other methods as Section \RomanNumeralCaps{6}-D on pages 22-24.}
% Our focus in the revised manuscript was to clearly state the novelties and contributions. We hope that you find the following response satisfactory. \\
\newline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{The authors can provide complexity and performance comparison of beam-surfer with beam-forecast, swift-link and HBA for a better exposition.}

Done. We have added this in two places: in Section II, lines 4-30 on pages 7, as well as added a new Section IX.D on performance comparison with other methods along several dimensions as Section IX.D on pages 22-24. We have also indicated a potential role for compressive sensing methods for determining a NLOS beam in Section \RomanNumeralCaps{1}-B, lines 13-15, pages 5. \\



\textbf{Can sampling strategies such as Thompson sampling in the spatial vicinity of currently selected beam be employed for beam selection to make the beam-adaptation/ exploration faster?} \\
 { Done, see Observation 2 in Section VII-B. For a uniform linear array, there are only 2 possible neighbors beams. For the case of a uniform planar array also there may be only two neighbor beams if the steering is only in the azimuth direction as in our testbed, and a maximum of 8 neighbor beams if steering is in both the azimuth as well zenith directions.
  So the search space is small, and we just use a simple method of testing the few possibilities and choosing the best as noted there. If there is a posterior probability distribution then Thompson sampling or other random exploration or learning methods can be used. Other approaches are compared in Section \RomanNumeralCaps{2}.\\~\\
  
 
  
\textbf{When both the optimal Tx beam involves a reflected path, i.e., in NLoS operation, how are better beams selected over time?   The optimal reflected beam can keep varying over time (with or without the LoS blocked). Why are 3dB and 10 dB chosen as thresholds in the protocol? What are the effects of tweaking these thresholds? } \\
Done. We have indicated in Section \RomanNumeralCaps{4}-D in lines 11-20 on page 15 that it is currently done by exhaustive search whenever the transmit beam changes, which we have found is sufficiently frequent to maintain a viable control channel, and that for further improvement one can also update each time the LoS receive beam changes, and to do so potentially using compressive sensing methods.
The reason for the 3dB threshold for
LoS is explained in Section \RomanNumeralCaps{4}-B, lines 8-12  on page 12.
% Reason for choice of 3dB threshold described in Section IV.A, page ??. For convenience we reproduce that here. ``For the main lobe of an antenna radiation pattern, the directional gain drops steeply after half power, hence 3dB gain is chosen to reflect this and to utilize a beam only within its beam width (half power points) where the gain is maximum. Also, the first null beam width, i.e, angular width between zero gain points for a linear array antenna pattern is approximately twice beam width. So the antenna gain drops steeply after the half power point."
The reason for the 10 dB threshold for NLOS is explained in Section \RomanNumeralCaps{4}-D, lines 20-26 on page 14.

% {\color{red} Professor, 10 dB threshold we use to detect blockage but here the lines suggest the why use a NLoS beam}
% As described in Section IV.B, page ??, the choice for NLOS was based on extensive experiments in indoor environments such as classrooms, corridors, and conference rooms in our building, where we found that the usable NLoS RSS is within 10 dB of LoS RSS.
% {\color{red} Can you add any other reason for the choice of 10dB other than that it was best in your experiments? If so, please add to the paper too.}



\textbf{What are the factors affecting BCT? How can it be bounded in general for indoor/outdoor channels?}\\ 
{Done. 
See Section \RomanNumeralCaps{4}-B, lines 17-19 on page 12.
% We have added the following in Section IV. Given a LoS path, a particular receiver beam can receive usable signal as long as LoS path remains within its receive beam width. 
% As the user moves, the LoS path moves out of beam width, and the duration after which the RSS drops below 3 dB from its maximum is the BCT. 
% So the primary factors affecting BCT are width of beam and user mobility. 
% Our experimental results for a 12 element phased array, presented in Section ??, pages ??-??, confirmed these are the main contributing factors in both indoor and outdoor channels. 
% Whether it is indoor or outdoor, communication requires either a LoS or NLoS path between Transmitter and Receiver. 
% Our observations present the empirical bounds observed for user mobility when a beam from 12 element phased array is used. It is hard to find general bounds as BCT depends on mobility, antenna orientation, beam width used. In our opinion, BCT should as seen as profile (like a Power Delay Profile, which varies from scenario to scenario) for a particular scenario but not as generic model based observation.  Also, we find such modelling as an interesting future problem and must be both exclusively and extensively studied.
\\~\\
\textbf{Given RSS vs time data, how is the BCT computed? What is the variance of the RSS within a BCT slot?}\\

Done. See Section \RomanNumeralCaps{4}-D, lines 30-31 on page 10 where it is explained how the
BCT is computed, and and lines 1-3  on page 11 for the standard deviation of the RSS within the BCT. 
% {\color{cyan}
% As described in Section IV.A, When the transmitter and receiver beams remain unchanged during a particular user motion pattern, duration over which received signal strength remains within 3 dB from the maximum is BCT. 
% 
% Variance of RSS within BCT depends on beam pattern within the half power beamwidths, which in turn depends on the type of array as well. RSS also depends on user motion pattern. Antenna radiation patterns often doesn't have closed form expression and researchers usually rely on numerical analysis. Variance of received signal strength, therefore is calculated based on observations. For simple translational motion and using 12 element phased array, variance is 1.2635
\\~\\
\textbf{The observations (such as on BCT and spatial correlation of beams) and conclusions drawn seem quite dependent on the channel geometry. How can this be generalized? In an outdoor channel geometry with multiple mobile scatters/obstructions, it is not clear why these observations and conclusions could remain valid. These observations and conclusions seem quite critical for the protocol's performance.} \\
{
% It is true that BCT is dependent on mobility and beam patterns. It is better to empirically calculate the same for a given system in similar fashion as power delay profile of channel in a given environment which vary from scenario to scenario. As we know a given power delay profile or channel model can’t be generalized so is BCT. Similar to channel parameters like delay spread which varies based on environment, BCT can only be characterized for particular system and mobility pattern. 
% 
% Our experiments in outdoor environment didn’t find usable NLoS path from scatterers, that is channel is primarily dominated by LoS path. For either a LoS path or NLoS path, we found BCT depends on beam width and user mobility, what we present in our work are experimental observations for typical motion patterns. Our protocol performance is independent of BCT durations, protocol can be tweaked based on BCT measurements for any intended mobility model and beam pattern, just like one of many empirical channel power delay profiles and neither of them can really replace others.
% 
Done. Please see the added paragraphs in Section \RomanNumeralCaps{4}-B, lines 13-19 on page 12.
% {\color{red}Santosh: Please point them to the location  with the lines ``Our results are based on experimental data collected over 2 months at different times of day,... empirically calculate BCTs for such scenarios to tune parameters of the protocol.}
% the same for a given system in similar fashion as power delay profile of channel in a given environment which vary from scenario to scenario. As we know a given power delay profile or channel model can’t be generalized so is BCT. Similar to channel parameters like delay spread which varies based on environment, BCT can only be characterized for particular system and mobility pattern. 
% 
% To the best of our knowledge, our work is the first in consolidating extensive experimental data for BCT for human walk. and we believe our observations of BCT stand as cross validation for the parameterizing BCT.
% We intend to release the data sets to the community for researchers to fit the data to identify a model. 
% However, we believe that is work in itself.
} \\

\noindent
\textbf{In Figs. 2a and 2b,  it is counter intuitive to notice that the RSS for D = 10m being always better than that of D = 5m, as one would expect the signal strength to drop with distance. Can this be reasoned?}\\
{Done. The reviewer is correct. The figures were earlier presented using different amplifier gains. We have now normalized all of them to use the same amplifier gain, and one can indeed see that RSS for 5m distance is indeed better than RSS over 10m distance.
% {\color{red} Santosh, I cannot understand this explanation? What is the y-axis of the graph? Can you please explain it to me orally? It needs to be rewritten to be succinct and super-clear.} We intend to present Fig 2a and 2b to reflect the change of RSS (not the absolute RSS) with time for a given motion pattern and distance than the true RSS. So, we adjusted receiver gains of our hardware to have similar RSS at 5m and 10m. We can either add text explaining the same or we present the true RSS mentioning the receiver gain employed at the distance and the TX power. Further, we request reviewer to consider the whenever we mention RSS not in absolute sense for the entirety of work, as we only focus on change in RSS.
}
\\~\\
\textbf{For a typical movement pattern, can the outage probability of beam-surfer be analytically characterized and rate guarantees be given?} \\
That remains a topic for future work.
It will require mathematical channel modeling, model of the environment, and mathematical modeling of motion including orientation of mobile, and will be an interesting topic for future theoretical work.
\\~\\
\textbf{It is not clear how the synchronization is performed in this setup.} \\
Done. This is explained in Section \RomanNumeralCaps{7}, lines 20-22 on page 25.
 

































==> reviewer3-3.tex <==
%\section{Response to Reviewer 3}
\textbf{Response to Reviewer 3}

{We thank the reviewer for the thorough review.\\
\newline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{How can a receiver know that the transmitted beam is misaligned?  Please clarify.}\\
{Done. A sentence is added in Section \RomanNumeralCaps{2}-A, lines 6-8 on page 4. 
% {\color{red} Please point them to the location where the sentences ``If neither of the beams $k-1$ or $k+1$ has a higher RSS, then the receiver requests the transmittter to try its neighboring beams." have been added.}
The details are indicated in Section \RomanNumeralCaps{5}, lines 6-12 on pages 17, as well as shown in the State Machine of Figure 5 for the node TBA (Transmit Beam Adaptation), and
the Flowchart of the protocol in Fig. 6 corresponding to TX Beam Adaptation.
% If the receive beam adaptation at user couldn't restore RSS within 3 dB then user requests Transmit beam adaptation.
}
\\~\\
\textbf{Considering the point 4 which is mentioned under the key experimental findings in page 11,
   authors should comment on the effect of error on the system performance, which may arise during
   refining the misaligned beams.} \\
 {In the extensive experimental evaluations conducted, in spite of all measurement and other errors, BeamSurfer is able to maintain received signal strength within 3 dB of what an Omniscient Oracle could possibly achieve in all the mobility scenarios studied. No algorithm can perform better than an Omniscient Oracle which always chooses the best beam, and so it is an absolute upper bound on performance, and generally unachievable. The maximum throughput loss compared to the oracle when signal strength is 3 dB lesser is around 30 $\%$.}
 \\~\\  
\textbf{ Is the presented beam management protocol, applicable for both TDD and FDD based
 systems? Authors please clarify this. } \\
 {The protocol is applicable for both TDD and FDD systems as it is based only on RSS.  We implemented protocol for TDD system.} 
\\~\\
\textbf{In the line 36 of page 26, it is written that “…..  schedules a set of beams with with ……. ”.
 Please correct this.} \\
{ Done}
\\~\\
\textbf{What will be the effect of imperfect channel state information on the presented beam
  management? Please clarify.} \\
  {BeamSurfer doesn't need channel state information as it only relies on received signal strength.} }










